Disclosure or Marketing? Analyzing the Efficacy of Vendor Self-reports for Vetting Public-sector AI

Documentation-based disclosure has become a central governance strategy for responsible AI, particularly in public-sector procurement. Tools such as model cards, datasheets, and AI FactSheets are increasingly expected to support accountability, risk assessment, and informed decision-making across organizational boundaries. Yet there is limited empirical evidence about how these artifacts are produced, interpreted, and used in practice. In this paper, we present a qualitative study of the GovAI Coalition FactSheet, a widely adopted transparency document designed to support AI procurement and governance in government contexts. Drawing on semi-structured interviews with vendors and public-sector practitioners, alongside a systematic analysis of completed FactSheets, we examine how FactSheets are used, what information they surface, and where they fall short. We find that FactSheets are asked to serve multiple and conflicting purposes simultaneously: showcasing vendor offerings, supporting evaluation and due diligence, and facilitating early-stage dialogue between vendors and agencies. These competing expectations, combined with the structural constraints of voluntary and public self-disclosure, limit the ability of FactSheets to function as standalone evaluation or risk-assessment tools. At the same time, our findings suggest that when understood as relational artifacts used to establish trust, shared understanding, and ongoing dialogue, FactSheets can help create conditions that support more meaningful disclosure and governance over time.

==> sections/1_introduction.tex <==
\section{Introduction}
Governments across the world are increasingly adopting Artificial Intelligence (``AI'') systems, with critical implications for the rights and safety of residents \citep{reisman2018algorithmic,kim2024public,chouldechova2018case,eubanks2018automating,whitney2021hci,kawakami2024studyingpublicsectorai,levy2021algorithms}. 
Within the United States, the site of this research study, FAccT scholars have studied how algorithmic design decisions embed value judgments and shape policy decisions for systems adopted within counties' social work \cite{eubanks2018automating,kawakami2022improving,gerchick2023devil} or criminal legal systems \cite{meyer2022flipping,pruss2023ghosting}.
Chronic lack of resources in the public sector \cite{johnson2025legacy} combined with recent shifts in both the availability and popularity of Generative AI adoption have intensified demand for AI tools within the public sector \cite{chen2025dispelling,johnson2025legacy}, as well as the urgency of establishing mechanisms for responsible oversight.

Meaningful oversight, however, is rarely straightforward. Understanding and intervening in the design of public sector AI systems is often complicated by the fact that the majority of these systems are not developed by government employees, but instead are purchased (or ``procured'') from private vendors \cite{mulligan2019procurement,rubenstein2020federal,hickok2024public,johnson2025legacy}. 
This reliance on third-party vendors creates legitimate barriers to governments' ability to meaningfully understand and govern the AI systems they purchase. 
These barriers surfaced by past research include vendors' claims of corporate secrecy \cite{pasquale2015black,brauneis2018algorithmic,kawakami2024studyingpublicsectorai}, governments' lack of access to technical talent \cite{mulligan2019procurement,rubenstein2020federal,engstrom2021artificially}, lack of participation in the technology design process \cite{veale2018fairness,mulligan2019procurement}, in addition to the general inscrutability and complexity of many modern AI systems \cite{lipton2017mythos,liao2024transparency}. 
These barriers are particularly difficult for smaller, under-resourced local governments to navigate \cite{johnson2025legacy}, resulting in structural information asymmetries that make it difficult for many organizations to independently assess risk, anticipate failure modes, or determine whether a given system is suitable for use.
% Softened: These structural information asymmetries often make it nearly impossible for governments to independently assess risk, anticipate failure modes, or determine whether a given system is suitable for use in local governments \cite{johnson2025legacy}. 

In recognition of these asymmetries between AI vendors and the governments they sell to, scholars and advocates have called for governments to play a more active role in interrogating AI systems and understanding the consequences of AI deployment \citep{mulligan2019procurement,richardson2019confronting,conti-cookguiding,rubenstein2021acquiring,hickok2024public,govai_openletter}. To this end, a variety of artifacts have been created to facilitate basic disclosures about vendor's AI systems, often operationalized as lists of questions for governments to ask of AI vendors during the procurement process ~\cite{wefbox,brauneis2018algorithmic,conti-cookguiding,dotan2023how}. 
One such prominent artifact widely adopted across local governments in the United States is the \emph{AI FactSheet} \cite{govai_factsheet}, developed and maintained by the GovAI Coalition, \bkedit{a collaborative effort among U.S. state and local governments seeking practical tools to govern AI adoption and share information~\cite{govai_openletter}.} The AI FactSheet consists of a list of 25 open-ended questions for public agencies to ask AI vendors, and invite vendors to disclose basic information about how their AI models were designed (\eg{} on what data, using which methods), and how they might perform in real-world contexts~\cite{govai_factsheet}. It has become a widely adopted and historically important mechanism for disclosure facilitation and information elicitation regarding vendors’ AI systems \cite{sharma2024power}. Over the past two years, the FactSheet has emerged as a default solution for many local governments in addressing information asymmetries during procurement, with more than 300 public-sector organizations and hundreds of vendors now using the tool in practice. The FactSheet has become a prime example and a case study for a broader class of documentation-based artifacts that are now central to AI governance regimes, from model cards \cite{mitchell2019model}, to transparency reports~\cite{bommasani2024foundation}, to algorithmic impact assessments \cite{moss2021assembling}. 

% Despite their increased adoption, little work to date has examined the effectiveness of these written documentation artifacts for enabling public servants to meaningfully understand and assess vendors' AI systems, and participate in AI governance. 
\bkedit{Despite their increased adoption, there has been little empirical examination of whether these written self-disclosure artifacts actually achieve the goals that advocates and scholars have articulated for them: aiding public servants in meaningfully understanding, assessing, and governing AI systems used in the public sector.}
More broadly, at present we lack a basic understanding of how existing written documentation artifacts are adopted in practice: what specific goals do governments have in requesting their completion, how vendors approach completing them, and what types of technical information vendors elect (or do not elect) to voluntarily self-report. \bkedit{Addressing this gap is essential for evaluating whether disclosure documentation fulfills its intended governance role, or whether structural and institutional factors limit what such artifacts can realistically deliver. To investigate these issues, we aim to answer the following research questions:
\begin{itemize}
    \item \textbf{RQ1:} What specific goals do public-sector agencies have when requesting the completion of AI disclosure documentation such as FactSheets?
    \item \textbf{RQ2:} How do vendors approach completing these documentation artifacts, particularly in the context of voluntary and publicly accessible disclosure?
    \item \textbf{RQ3:} What types of technical, evaluative, and governance-related information do vendors elect to voluntarily self-report, and what information is consistently limited, generalized, or omitted?
\end{itemize}
}
In this work, we conduct a novel mixed-methods empirical study to evaluate the efficacy of the GovAI FactSheet in allowing public-sector agencies to vet AI solutions. FactSheets serve as an important case study of documentation more broadly as a means of encouraging developers to provide transparency, and subsequently, imposing accountability for their AI products and services. 

To understand how key stakeholders approach and use the FactSheet, we conducted over 20 hours of qualitative interviews with both AI vendors and public sector workers. We complement our findings from these interviews with a review of all of the completed AI FactSheets available to GovAI Coalition members as of October 2025, analyzing 43 completed FactSheets of 43 real AI systems which are currently sold to U.S. local governments. These findings have been informed by privileged access across months of embedded participant observation within the GovAI Coalition attending workshops, observing inter-agency working groups, and tracking the day-to-day evolution of FactSheet practices. This combination of data sources allows us to understand both how stakeholders conceptualize the purpose of documentation and what kinds of disclosures documentation actually produces.

% Our analysis reveals key tensions in how different stakeholders envision the purpose of existing documentation artifacts. Working alternative below:
\bkedit{Our analysis reveals that there is tension when FactSheets try to simultaneously fulfill the evaluative and governance roles often expected of them, in large part because different stakeholders approach these documentation artifacts with competing and sometimes incompatible goals.}
Governments often request FactSheets to support procurement due diligence, risk assessment, or legal compliance. Vendors, on the other hand, frequently view them as marketing tools, opportunities to shape impressions, or obligations to be met with minimal risk. These competing orientations produce substantial gaps between the intended and actual uses of documentation. 
% As a result, we illustrate how many of vendors' responses to AI FactSheets fail to disclose basic information about how AI systems are designed (such as [example info]), or, in some cases, may even mislead public sector workers by giving them a false sense of assurance.
\bkedit{These differing approaches create a mismatch between what governments expect documentation will provide and what vendors feel able or incentivized to disclose. As a result, many FactSheets lack the system design, evaluation, or governance details needed to meaningfully support public-sector decision making.}

% Our research contributes to a deeper understanding of the role that self-disclosure by vendors can play in facilitating the assessment of AI systems within the context of existing relationships between stakeholders. Alternative below:
\bkedit{Our findings suggest a fundamentally different way to understand the role that self-disclosure documentation can play in facilitating the assessment of AI systems within the context of existing relationships between stakeholders.}
Our qualitative findings reveal how vendors' willingness to share information with public agencies is shaped by a larger backdrop of challenges that vendors and governments face when communicating with each other throughout the procurement process. Vendors’ willingness to disclose meaningful information is shaped by fears of reputational harm, concerns about legal liability, uncertainty about how information will be interpreted, and a lack of incentives to invest in detailed responses. Governments, for their part, often lack the power, expertise, or contractual leverage to require more informative disclosures. These conditions create a fundamental limitation to the efficacy of documentation mandates, even when they are broadly adopted. 

% This grounded, relational understanding of self-disclosure artifacts illustrates how they can still play an important role in opening up continued conversations about vendors' AI systems, even if the information they provide is incomplete. We argue that when documentation is understood as part of a relationship rather than a standalone artifact, its value shifts away from final decision-making tools toward a process for fostering healthy collaboration through trust and communication. Understanding the problem of meaningful disclosures within this broader context of ongoing communication and relationship-building between stakeholders also enables us to explore alternative solutions that take existing relational challenges into account.
\bkedit{This grounded, relational understanding of self-disclosure artifacts proposes why FactSheets may fall short as standalone tools for AI assessment, but still play an important role in opening and structuring ongoing conversations about vendors’ systems. When documentation is understood as part of a relationship rather than a final evaluative artifact, its value shifts away from enabling one-time decisions and toward supporting trust, shared understanding, and iterative engagement. This reframing does not abandon the original goal of facilitating meaningful assessment. Instead, it suggests that assessment is more likely to be achieved through layered governance processes in which FactSheets serve as an entry point. Situating disclosure within this broader context of ongoing communication and relationship-building allows us to explore governance approaches that better align with how information is produced, shared, and acted upon in practice.}

% I don't know if I understand this one. 
In summary, our paper contributes a critical perspective on vendor self-reporting documentation by surfacing the larger relational challenges that limit AI vendors from sharing information about their AI systems. We argue that many existing documentation artifacts, which rely on voluntary written disclosures from vendors, are subject to key failure modes that may often render them ineffective at supporting meaningful oversight over vendor's AI systems. We hypothesize that these limitations may be widely applicable to similar disclosure documentation artifacts which have been proposed as a key component of other AI governance regimes \cite{}. We conclude by providing reflections and speculative recommendations for how future research might support meaningful cross-stakeholder disclosures, and outline constructive pathways for designing disclosure mechanisms that better reflect the realities of procurement, including clearer purpose alignment, differentiating audiences, and creating better incentive structures that reward meaningful disclosure rather than superficial compliance.


==> sections/6_recommendations.tex <==
\section{Recommendations}

==> sections/old_4-1.tex <==
\subsection{Analyzing vendor's completed self-disclosures}
In this section, we examine how vendors complete AI FactSheets in practice. Our analysis of the full corpus of completed GovAI FactSheets reveals a consistent pattern: while vendors generally provide relevant and coherent responses to each prompt, those responses frequently omit basic technical details about system design, training data, and performance. As a result, many responses gesture toward disclosures without rendering the system itself legible to a reader seeking to understand how the AI system was built, or how it performs.

\begin{wrapfigure}{r}{0.5\linewidth}
    \includegraphics[width=\linewidth]{source//figs/CDT_scores.pdf}
    \caption{While vendors frequently provide meaningful information about intended use and contextual limitations, disclosures relevant to evaluation, governance, and training data remain sparse. This asymmetry underscores the mismatch between expectations that FactSheets function as evaluation tools and the realities of voluntary, public-facing documentation, reinforcing their practical role as relational, early-stage governance artifacts.}
    \label{fig:rubric_scores}
\end{wrapfigure}

As a first step towards characterizing how the quality of information reported by vendors varied across the entire dataset of available factsheets, we scored each factsheet using the CDT's recently published rubric for assessing transparency in the public sector. 
Figure \ref{fig:rubric_scores} summarizes aggregate scores across four dimensions: use and context limitations, governance structures, training data, and evaluation and testing. We provide the complete rubrics and scoring criteria for each dimension of disclosure in Appendix \ref{app_methodology}, and show example rubrics for training data disclosures and performance metrics in Table \ref{tab:training_data_disclosures} and Table~\ref{tab:performance_metrics_disclosures}, respectively.

Vendors received the highest scores when reporting use and context limitations, and received the lowest average scores for reporting their training data and evaluation.
The use and context dimension aims to measure whether a factsheet can ``\emph{clearly articulate what [the vendor's] tool should be used for}'' by providing information about the specific tasks and business use cases the AI system can support.
Indeed, many factsheets provided clear statements of intended use, such as a ``product that uses AI to run code checks by users within a city's permitting department'', or an object detection system designed to ``detect blight such as housing code violations or graffiti''.
These responses clearly articulated an intended user of the system and the type of labor that vendors intended their AI to support or automate.

In contrast, vendors' disclosures about governance, training data, and performance received much lower scores. In these categories, the majority of vendors received the lowest possible score, indicating that ``little to no relevant information'' was provided.
For example, even when explicitly prompted on the FactSheet to disclose ``\emph{any relevant information, links, or resources regarding your organization's responsible AI strategy}'', many vendors left the field blank, supplied broken links, or described that developing an AI governance policy was still ``in progress''.
Because training data and evaluation are foundational to assessing bias, reliability, and fitness for use, and because they were the lowest scoring dimensions, we focus the remainder of this section on the variation and gaps in vendors’ disclosures along these two axes.

\xhdr{Unpacking vendors' training data disclosures} The FAccT community has long recognized that training dataset curation plays a critical role in shaping AI system behavior \cite{bender2018data,Gebru2021,pushkarna2022datacards}. 
Within the public sector, scholars have documented how training data disclosures are a key site for assessing biases encoded by dataset practices \cite{gerchick2023devil,hickok2024public}, validity concerns \cite{coston2023validity}, and dataset shift \cite{mulligan2019procurement}, especially because vendors often do not design or train bespoke AI systems for each locality, and instead deploy the same systems across multiple local contexts \cite{veale2018fairness,kawakami2024studyingpublicsectorai}.
%Within a public procurement context, scholars have written about how training data disclosures operate as a key site to facilitate more informed reflection on potential societal biases, questions of validity, and risks of dataset shift \cite{veale2018fairness,coston2023validity,hickok2024public}.
%Public-sector training data disclosures are particularly essential given that the vast majority of vendors do not design or train bespoke AI systems for each government, and instead deploy the same AI system, off-the-shelf.
Not least, this work is situated within a larger backdrop of concerns from public sector workers about whether the datasets underlying modern generative AI systems were obtained legally, and with consent \cite{rueter2024want,johnson2025legacy}. In what follows, we describe what types of technical information vendors do and do not provide in their FactSheet responses about their training datasets.

In analyzing the contents of vendors' training data disclosures, we found that most responses lacked the information needed to form a basic understanding of what data was collected. This pattern is reflected in the large share of responses that received a rubric score of 1, indicating that little to no description of the training dataset's contents was provided (Table \ref{tab:training_data_disclosures}). Vendors in this category offered only minimal or generic statements, such as that a dataset was ``collected with proprietary methods'' [FS8], that a model was ``trained by customer staff'' [FS9], or was trained using ``tens of thousands of images'' [FS10], without specifying what those data actually were. In many cases, disclosures provided boilerplate language that was so general that it could apply to nearly any AI system, such as statements that generative AI systems were trained on ``large, diverse, open-source datasets curated from the Internet'' [FS21].

A smaller subset of responses offered more insight into the shape and contents of vendors' datasets, and thus were assigned a score of 2. Disclosures within this category provided enough detail to understand the type of data that was collected, such as a description that a resident-facing chatbot was trained on ``publicly available government webpages'' (Table \ref{tab:training_data_disclosures}), or that a tool to review permitting applications was trained on ``historical project files shared by the permitting departments of municipalities.'' Still, many such disclosures rarely specified how these data were obtained, or which populations they represented, such as \emph{which} municipalities contributed these documents. As a result, the provenance of many vendors' datasets, and their relevance to practitioners' own context, remains difficult to understand and assess.

%Beyond uncertainty about what data were used, we also observed substantial ambiguity about whether vendors were ``training'' their systems at all. This challenge reflects a growing trend of public sector AI vendors' increasing reliance on large pretrained foundation models, which can be deployed either with or without additional training (\eg{} using methods such as supervised fine-tuning or in-context learning \cite{oai_sft,mosbach2023few}).While some vendors explicitly stated that they ``did not train any AI systems'' and instead deployed off-the-shelf models (\eg{} OpenAI or Microsoft Azure), other vendors' responses left their practices unclear. For example, one internal productivity chatbot reported that they ``train their system using customer-specific datasets containing public records and zoning documents'', but did not specify whether these data were used to train a bespoke model, or merely provided as context for a RAG system.

%Such disclosures left the system’s actual mode of customization opaque.


%While some vendors reported using these models without modification, others described incorporating customer-provided datasets through mechanisms such as RAG or in-context learning. 
%Yet disclosures rarely clarified how these data were used, leaving it unclear whether they shaped model behavior through training, fine-tuning, or merely contextualization.

\xhdr{Unpacking vendors' reported performance evaluations} FAccT scholars have long characterized how AI systems are susceptible to ``fallacies of functionality'' where they do not always work as advertised \cite{raji2022fallacy}, a key concern for public-sector AI systems used in safety-critical contexts such as influencing sentencing decisions \cite{pruss2023ghosting} or generating police reports \cite{adams2024no}.
AI procurement scholars have discussed how performance evaluations can allow governments to assess the capabilities and limitations of individual AI systems, while also gaining a realistic sense of what AI can achieve across public sector contexts, enabling public sector workers to make more informed procurement decisions \cite{rubenstein2020federal,johnson2025legacy}.
To this end, the GovAI factsheet `Performance Evaluation' prompt asks vendors to report both how they measure performance, and their ``current level of performance on these metrics''. 

When we analyzed vendors' performance evaluation disclosures, we found that vendors' free text responses varied considerably from each other, reflecting high variance in how performance is conceptualized and measured across different public sector applications and domains. 
%In this section, we describe trends in the amount of technical information that was or was not disclosed. 
As a shared framework to assess the amount of information that was reported, we adopt \citet{raji2021aiwideworldbenchmark}'s conceptualization of AI performance evaluations as a combination of a dataset of instances, and a metric that describes how success is measured. This framework clarifies the information that is needed to interpret vendor's performance claims \cite{liao2021are}.

Across the corpus of FactSheets, vendors' responses varied in the amount and specificity of performance information they disclosed. Notably, over half of the FactSheets did not report \emph{any} performance evaluation result, receiving the lowest rubric score (Figure~\ref{fig:rubric_scores}). While many vendors provided at least some description of how they conceptualized performance, these descriptions often remained underspecified: for example, stating that the vendor measures the ``accuracy'' [FS28] or ``usefulness'' [FS1] of system outputs without defining how these concepts are operationalized and measured. Some vendors referenced concrete metrics, such as a vendor that stated that their evaluated their translation system by using BLEU scores and Word Error Rate, but did not report any corresponding evaluation results.

    A smaller subset of FactSheets did contain performance results, reported as aggregate metric scores (\eg{} ``Our system achieves 95\% accuracy''[FS36]). However, these disclosures rarely included information about the datasets used to calculate the reported scores. Vendors either provided metrics without any dataset description, or stated that evaluations were conducted using ``internal''  [FS13] or ``proprietary'' data  [FS19] (\eg{} ``90\% response accuracy based on internal testing''), with no further details about the contents of these datasets. 
Critically, none of the reported performance evaluations were reported using publicly available datasets, making numeric performance results difficult to contextualize and interpret.

\xhdr{Summary} Our analysis of completed FactSheets offers one of the first empirical accounts of how AI vendors respond to requests for basic disclosures about their AI systems. Although such disclosures are often framed as a way for governments to gain insight into vendors' value-laden AI design choices \cite{}, our analysis shows that vendors share little concrete information about training data or performance evaluations. Across the dataset of FactSheets, basic information such as from where data was obtained, or how a system performs, is frequently missing or underspecified, leaving key aspects of system design and its capabilities and risks opaque. The consistency of these patterns across vendors motivates our interest in understanding the broader incentives and constraints shaping vendor disclosures.
\njcomment{TODO add citations here: related to the lit review todo}


\xhdr{FactSheets as showcasing value added} Across interviews with both vendors and public-sector practitioners, one common way of understanding the FactSheet was as an opportunity to showcase the value an AI system provides for a particular public sector use case or application. Rather than framing the document primarily as a vehicle for providing detailed technical descriptions, many participants described it as a space for vendors to communicate their AI system's benefits, differentiation, and practical relevance.

%This orientation toward showcasing value was visible both in how stakeholders discussed the FactSheet and in how vendors completed it in practice.

When asked what they saw as the value and motivations for completing the FactSheet, interviewed vendors frequently characterized the FactSheet as a way to highlight what makes their system attractive in a competitive market. One vendor participant emphasized wanting ``more opportunity to showcase what differentiates [our] product from the competition,'' [VP3] while another framed the FactSheet as a way to gain ``any exposure, especially for small companies,'' [VP1] explaining their desire to ``maximize the eyeballs'' that ultimately see it. 
This hope was a direct consequence of the dataset of completed FactSheets being made public and searchable by the Coalition, as a ``marketplace'' for customers to browse and select between potential AI offerings.
Within this context, vendors were aware that their FactSheet may be a potential customer's first introduction to their product or service.
This understanding of the FactSheet as primarily articulating the business value of an AI system was not limited to vendors. 
Agency interviewees often echoed similar priorities, emphasizing outcomes and problem-solving over what they perceived as unnecessary technical aspects of system design. As phrased by one public-sector participant: ``We don't want to get technical about how [the AI] works. I don't care about the programming, or what program you use, but how does it solve the problem?'' [AP2]

Across the completed FactSheets, vendors’ responses frequently emphasized the value and fit of their services rather than providing substantive technical disclosures. Beyond outlining intended use cases, vendors often framed their systems using language that foregrounded anticipated benefits, such as efficiency, innovation, and alignment with public-sector values. This trend was reflected in the largely positive and promotional language that vendors used to describe their products, such as statements that vendors' AI systems would ``\emph{revolutionize} government operations'' [FS4], ``help municipalities \emph{maximize efficiency}'' [FS29], or ``offer always-available, tireless, and patient support'' [FS16] (emphasis is added by us). This orientation extended beyond vendors' product descriptions to include other types of assurances about system design or regulatory compliance. Many of these assurances were often framed as vendor-managed concerns, such as assurances that ``all training is done on publicly available data''  [FS39], that updates occur ``frequently''  [FS1], or broad commitments to ethical values, \eg{} a vendors' commitment to ``thoughtful design [that] ensures you can use AI safely, responsibly, and ethically''  [FS3]. The prevalence of highly positive descriptions of system capabilities and value-aligned commitments suggests that many completed FactSheets might be designed to produce a favorable impression of vendors’ AI systems.

This showcasing orientation was also evident in how vendors interpreted and framed their responses to underspecified factsheet prompts. For example, in response to an open-ended prompt to disclose performance evaluations, several vendors reported metrics that emphasized their system's capabilities and business value, such as claims their system enabled a ``70 to 90 percent reduction in report-writing time''  [FS18], or the ability to ``reduce [task completion] to around 2-7 minutes''  [FS18]. While such metrics may be meaningful to prospective purchasers seeking to understand a system's potential benefits (\eg{} to gain internal buy-in within their city), they differ from the technical performance evaluations (\eg{} of system accuracy, bias, or robustness) typically expected in AI evaluations. This emphasis on benefit-oriented reporting is further reflected by the absence of evaluations that would surface system limitations, or potential societal harms.

%To summarize, many FactSheets would serve this goal well, echoing this vision we heard from many vendors that they approached the FactSheet as an opportunity to articulate the value of their service (make this seem less mean and more like they're just entrepreneurs trying to survive).


==> sections/old_discussion.tex <==
\section{Old Discussion}
(Preamble)

\subsection{Unpacking the affordances and limitations of voluntary vendor self-disclosures}
Our qualitative findings and rubric-based assessment suggest a need to reconsider how factsheets are conceptualized within public-sector AI governance. Figure~\ref{fig:rubric_scores} highlights a pattern that surfaced repeatedly in interviews. 
While factsheets often contain relatively informative descriptions of intended use and contextual limitations, they provide far less information about evaluation practices, governance structures, and training data. This unevenness is not a failure of vendors to comply, or a failure of the GovAI factsheet itself, but it is evidence of a potentially deeper mismatch between the expectations placed on documentation and the structural conditions under which it is produced.

A common interpretation implicit in most transparency frameworks is that factsheets can function as standardized artifacts to allow comparison, risk assessment, and quality judgments across systems. 
But, our interviews suggest that this expectation is difficult to realize in practice. Voluntary, publicly accessible self-disclosures are constrained by legal risk, competitive pressure, upstream dependencies (e.g., foundation models), and limited organizational visibility. 
This can create a space where written artifacts can then be used as an illusion of visibility without providing the verifiability that responsible governance requires. 
The rubric scores underscore this point. Dimensions most closely associated with evaluative rigor consistently receive lower scores, even when vendors engage in good-faith completion. 

% I would weaken this hypothesis: "We theorize that other governance regimes that similarly rely on voluntary self-disclosures may face similar structural obstacles [...]."
\bkedit{Seen in this light, the limitations observed are not shortcomings of this particular factsheet initiative, but may be structural obstacles faced by documentation-based governance efforts more broadly.
We theorize that similar challenges may arise wherever public-sector oversight relies primarily on voluntary self-reporting as a proxy for deeper evaluation, particularly in complex and rapidly evolving technical domains.}

% \xhdr{Why Factsheets Face Obstacles as Evaluation Tools}

% This is one of the strongest paragraphs in the discussion. I kind of want to be able to emphasize and thicken it
Viewed specifically as evaluation mechanisms, factsheets face structural challenges that can make them ill-suited to support meaningful disclosure on their own. Their voluntary nature may limit the completeness and comparability of disclosures, while their public visibility discourages honest acknowledgement of risks, failures, or known limitations. 
The presence of narrative prompts may further complicate attempts at consistent comparison across vendors, and vendors themselves often lack the information needed to provide detailed responses about upstream or foundation model characteristics. Taking these factors collectively may mean that relying on factsheets for risk assessment can skew expectations with what the format can realistically deliver.

This does not mean that evaluation is unimportant, but that expecting a single, public-facing document to bear that burden may be unrealistic. Treating factsheets as if they should succeed as evaluation tools risks misdiagnosing the problem and proposing solutions that may overemphasize better prompts or stricter guidance while leaving underlying incentive structures unchanged. 

% I think we can be even more concrete here about the recommendation and targeted audience. It seems like the key take-away is something like: Given the limitations we've surfaced of the ability of voluntary self-disclosures to facilitate meaningful evaluation, we believe that other, complementary interventions -- such as independent evaluations -- are urgently needed to support public servants in making sense of what they're buying. (you can include the lines here about future research for FAccT)
For policymakers and procurement professionals, the implication is concrete; visibility through documentation should not be mistaken for verifiability or rigor. Effective evaluation requires layered processes that combine written artifacts with interactive or empirical methods, including third-party audits, structured testing, scenario-based assessments, or standardized procurement checklists. 
% We argue that this highlights opportunities to explore alternative evaluative methods such as secure disclosures, collaborative testing protocols, or tiered information-sharing frameworks that might complement or even surpass documentation-based governance. These ideas point toward promising avenues for future FAccT scholarship and practice.
For the FAccT research community, this finding highlights the need to design and study complementary governance mechanisms that help public servants make sense of what they are buying, rather than relying solely on vendor-authored disclosures. Exploring secure disclosures, collaborative evaluation models, or tiered information-sharing frameworks represent promising directions for future research and practice.

\subsection{An Interpretive Shift: Seeing transparency documentation as a relationship, not compliance}
% Feedback: This needs to be workshopped. It might be tempting to see these documents as a one-and-done to facilitate compliance (maybe cite literature that might perpetuate this belief? or just the basic notion of "ask for it to be completed, hand it back") But it's really just the beginning of a longer conversation

A more productive interpretation, and one that aligns closely with how factsheets are actually used in practice, is to view them as relational infrastructure. 
From this perspective, factsheets function less as repositories of definitive information and more as mechanisms for structuring early-stage dialogue, surfacing assumptions, and establishing the terms of engagement between vendors and public-sector actors. This framing helps explain why use and context-related information is more consistently disclosed. These details may often feel less risky to share publicly and more immediately useful for determining relevance and fit.

The value of the GovAI factsheet lies in its ability to initiate longer-term relationships in where questions of quality and risk can be explored through additional, more appropriate channels. 
This relational framing resonates with broader FAccT scholarship that critiques performative transparency[ref] and emphasizes disclosure by design[ref], procurement as policy[ref], and the limits of documentation divorced from institutional process[ref].

Importantly, this interpretive shift does not diminish the ambitions of initiatives like the GovAI Coalition. Instead, it reframes their contribution so that factsheets can succeed precisely by not trying to do everything at once. 
When positioned as conversation starters rather than evaluative endpoints, they align more closely with both vendor constraints and agency needs.


If factsheets are best understood as relational tools, the question becomes how governance ecosystems can better support that role. 
This requires aligning incentives so that meaningful disclosure is rewarded rather than penalized. Today, many of the disincentives identified in our findings such as legal exposure, competitive risk, and unclear downstream use, remain largely unaddressed. As a result, even well-designed transparency initiatives struggle to develop the kinds of information policymakers hope for.

One implication is that evaluative information should increasingly be shared through complementary mechanisms rather than public, voluntary documents alone. These might include secure or non-public disclosures, third-party or joint evaluations, sandboxing environments, or tiered information-sharing processes linked to system risk and procurement stage. Within an ecosystem like this, the factsheet can play a critical role by helping to coordinate when deeper assessment is needed and which follow-on processes are appropriate.

Incentives are central to this shift. Higher-quality disclosures could be encouraged through tangible benefits such as expedited procurement review, preferred access to pilot programs, enhanced visibility within trusted registries, or clearer pathways to long-term vendor relationships. Importantly, these incentives should be matched to the factsheet’s intended function as rewarding openness that supports productive engagement rather than penalizing vendors for the inherent limits of public disclosure.






\subsection{Interpreting the Findings} 
\subsubsection{Implications for Transparency and Governance Research}
Our findings suggest that, as one case study of transparency artifacts used in public-sector AI governance, GovAI factsheets play multiple roles at once, often without an intentional design strategy that accounts for their competing functions. We suggest that transparency scholarship within the FAccT community should shift attention and effort from documentation content alone toward exploring documentation function. Rather than treating transparency documents as neutral repositories of information, our analysis illustrates how they operate as relational tools embedded within procurement workflows, institutional constraints, and vendor-government dynamics. This relational framing helps explain why content quality alone is an incomplete measure of governance effectiveness and why documentation can only partially support the aims of technical evaluation, institutional trust-building, and public accountability.

\subsubsection{Reconciling the Multiple and Conflicting Purposes of Factsheets}
Across our interviews, factsheets emerged as serving three simultaneous but conflicting purposes: showcasing vendor offerings, enabling preliminary evaluation, and supporting early-stage conversation. Vendors, for example, rely on factsheets to communicate value and differentiate themselves, while managing the risks associated with public disclosure. Agencies, by contrast, often hope to use the same document as a basis for comparability, due diligence, and early risk assessment. These expectations collide with the promise of the factsheet itself as a universal template that invites general narrative responses rather than the specificity agencies often seek. The fact that factsheets are both voluntary and publicly accessible further discourages full risk-related disclosure and allows for strategic completion that emphasizes strengths and avoids sensitive details.

These tensions make clear that a single artifact cannot effectively serve all three purposes. Expecting a factsheet to function simultaneously as marketing media, an evaluative instrument, and a risk-disclosure tool strains its design and erodes its usefulness. This has important implications for governance frameworks. We argue that researchers and policymakers should avoid conflating these aims and should instead select and institutionalize a primary purpose for factsheets. Once a central purpose is identified, the format, workflow placement, and incentive structures surrounding the factsheet can be redesigned to support it, rather than forcing one document to satisfy competing demands.

\subsubsection{Rethinking Transparency and Documentation Artifacts}
A key interpretive shift emerging from this study is that transparency artifacts should be viewed not as standalone disclosures but as relational mechanisms that structure communication across organizational boundaries. The effectiveness of a factsheet is shaped less by the completeness of its answers and more by the way it facilitates the interaction between vendors, procurement officers, and broader governance institutions. This perspective applies equally to model cards, risk assessments, impact statements, and other documentation tools whose value lies in how they position actors within a communication ecosystem, prompt clarifying questions, or help elicit shared expectations.

Our findings also underscore the limitations of documentation as a foundation for technical or risk-based evaluation. Vendors may lack visibility into upstream components, rely on foundation models they cannot fully characterize, or face legal and reputational constraints that limit what they can share publicly. Written artifacts can then create an illusion of visibility without providing the verifiability that responsible governance requires. Policymakers should therefore treat transparency documents as inputs into dialogue and verification, rather than as sufficient evidence for evaluation. This implies a need for complementary governance processes that combine conversation, testing, auditing, and empirical assessment with the interpretive function of documentation.

\subsubsection{Why Factsheets Fall Short as Evaluation Tools}
Viewed specifically as evaluation mechanisms, factsheets face structural challenges that make them ill-suited to support meaningful disclosure. Their voluntary nature limits the completeness and comparability of disclosures, while their public visibility discourages honest acknowledgement of risks, failures, or known limitations. The presence of narrative prompts further complicates attempts at consistent comparison across vendors, and vendors themselves often lack the information needed to provide detailed responses about upstream or foundation model characteristics. These factors collectively mean that relying on factsheets for risk assessment skews expectations with what the format can realistically deliver.

For policymakers and procurement authorities, the implication is that visibility through documentation should not be mistaken for verifiability or rigor. Effective evaluation requires layered processes that combine written artifacts with interactive or empirical methods, including third-party audits, structured testing, scenario-based assessments, or standardized procurement checklists. For the research community, these findings highlight opportunities to explore alternative evaluative methods such as secure disclosures, collaborative testing protocols, or tiered information-sharing frameworks that might complement or surpass documentation-based governance. While these ideas remain exploratory, they point toward promising avenues for future FAccT scholarship and practice.

\subsection{Recommendations for policymakers and governance researchers}
\subsubsection{What Factsheets Are Useful For: Implications of the "Relationship Building" Role}
Despite their apparent limitations as evaluative tools, we see that factsheets demonstrate value as relational instruments early in procurement to facilitate conversations between stakeholders. They help agencies articulate needs, assumptions, and constraints in accessible language, while giving vendors a way to signal relevance without having to over invest time and effort in extensive documentation at the beginning. When we frame the factsheet as a low cost/effort mechanism for initial and continued scoping, it can help everyone involved determine when to invest in further collaboration and when goals are not aligned. 

To function in this conversational role, factsheets require clear expectation-setting and thoughtful/effective integration into procurement workflows. Agencies need a shared understanding of what the factsheet can and cannot do, and should position it within early procurement stages, heavily relying on it during [I don’t know the official names of the stages, but like pre-RFI, during the pre-bid, etc], rather than treating it as a formal technical evaluation document. Clear guidance on appropriate follow-up steps, such as sandboxing, structured demonstrations, or technical assessments, can help the factsheet serve as a launching point rather than an endpoint.

This suggests a broader policy shift where factsheets should be formalized as pre-procurement dialogue tools rather than risk assessment instruments. Doing so would better align their actual strengths with organizational needs. Modular or purpose specific templates could improve this alignment, such as creating a core conversational factsheet that is supplemented by optional evaluative modules or procurement stage specific portions. Structured short-answer formats could also improve consistency and participation without overburdening vendors.

\subsubsection{Recommendations for future research: More speculative, forward-looking reflections on how we might address some of these limitations: Develop alternative channels for evaluative information, and incentivize good behavior}
Looking forward, we believe that improving AI procurement governance will likely require innovations that extend beyond documentation. Alternative channels for obtaining evaluative information such as secure, non-public disclosures, third-party or joint evaluation processes, or tiered requirements linked to system risk, may help address the structural limits of public, voluntary documents. Aligning incentives is equally critical. High-quality disclosures could be rewarded through privileged access to high visibility demonstration opportunities, expedited review processes, or visibility within public registries, depending on the intended purpose of the documentation. Concrete benefits to thorough disclosure can help governance bodies shift the status quo toward more meaningful transparency. 

Together, these innovations point toward a nuanced evaluation ecosystem that recognizes the value of documentation while also addressing its intrinsic limits. Factsheets can play a productive role within this broader system by facilitating early dialogue and supporting relational trust-building. Realizing their full potential requires clearly defining their purpose, aligning institutional incentives, and pairing them with complementary evaluation processes capable of upholding the standards that responsible AI procurement demands.


==> sections/old_findings.tex <==
\section{Findings}
Across both our interview analysis and our review of completed factsheets, we found that the approach stakeholders take for the factsheet is shaped by the broader goals and incentives they face throughout the procurement process. Vendors, agency staff, and other organizations bring different expectations to the document which are tied to institutional pressures, strategic aims, and practical constraints. As a result, the factsheet ends up serving multiple, sometimes competing purposes.

Stakeholders in our sample approached the factsheet with diverging goals. For many, completing the factsheet was intertwined with the goal of showcasing a product where they expect to demonstrate capability, credibility, and viability in a competitive market. For others, the factsheet was often viewed through the lens of evaluation where it was viewed as a tool for assessing what is being bought and whether a system is suitable, trustworthy, or compliant. And for both groups, the factsheet frequently functioned as a way to start building productive long term relationships where it acts as a procedural mechanism to align expectations early, structure discussions, and negotiate feasibility during procurement or pilot scoping. These divergent expectations are compounded by the multiple institutional functions attached to the document such as governance requirements, procurement artifacts, discovery tools, and marketing assets.

We argue that these differing goals are not only stated in interviews but that they are reflected in the ways the examined factsheets were completed. To analyze this, we take the perspective of the reader and ask “How well do the factsheets, as written, serve each of these goals?” Overall, we observed that factsheets are often worded in ways that lend themselves toward showcasing and relationship building, and less often as a means for effective technical evaluative transparency. We would like to acknowledge that for this analysis, while we assess how suitable the factsheets would be for each of these goals, we do not claim to assume the intention of the vendors that filled them out. 

The remainder of this section proceeds in two parts. First, we outline the broader goals and expectations that shape how stakeholders conceptualize transparency documentation in procurement contexts. Second, we examine the extent to which the completed GovAI factsheets can meet these expectations, identifying where the document format aligns with stakeholders’ needs and where it falls short.

Across this analysis, a central tension emerges. The goals of marketing, meaningful evaluation, and early-stage negotiation pull the factsheet in different directions. A single artifact rarely satisfies all three simultaneously. While factsheets are frequently highlighted in policy and governance frameworks as tools for verification, risk assessment, and accountability, our findings indicate that in current practice they are not well suited as standalone instruments for robust performance assessment or technical scrutiny.

At the same time, factsheets are far from irrelevant. When understood relationally (read as conversation infrastructures embedded in procurement workflows) they support critical early scoping functions and help stakeholders establish shared understanding. Their value lies less in offering definitive, evaluable detail and more in fostering structured communication. In the sections that follow, we unpack how these goals manifest and the implications for AI assurance, transparency policy, and procurement practice.

\subsection{Multiple and competing purposes of the factsheets}
Our interviews revealed that stakeholders do not share a single understanding of what a factsheet is for, and don’t have a shared picture of who its primary audience should be. Instead, the factsheet sits at the intersection of multiple institutional pressures to include procurement requirements, vendor success in competitive markets, expectations for responsible AI oversight, and the pragmatic need to build relationships early in the procurement process. As a result, stakeholders approach the factsheet with distinct and sometimes competing goals, namely solving a problem, enabling meaningful evaluation, and initiating dialogue. In the following subsections, we unpack each of these goals. For each goal identified in the interviews, we present how stakeholders described its purpose and how the completed GovAI factsheets support that purpose in practice.

\xhdr{Factsheets as showcasing value added}
One major function of the factsheet that was present in many of our interviews across all stakeholder groups was that it is an opportunity to demonstrate the value of a system for a given problem. In other words, both groups have a desire to communicate and understand the potential value and benefits that arise from applying a given system to a particular AI use case. 

\textit{Interviews} This sentiment was present in nearly every vendor interview. For example, one participant shared their desire for “more opportunity to showcase what differentiates [our] product from the competition.” and another expressed that they wanted to find “any exposure, especially for small companies. So I look for those opportunities to be able to "maximize the eyeballs" that ultimately see it.” But surprisingly, this was a common sentiment among agencies as well. For example, we talked with one government employee who said: “We don't want to get technical about how [the AI] works. I don't care about the programming, or what program you use, but how does it solve the problem” - AP. 

For many, this alignment-based orientation was not about deception, but about fit. These approaches highlight system features in language that is accessible to non-technical audiences, and strive to convey the benefits and improvements that an agency can expect when implementing a particular system. 

\textit{Documentation}
Accordingly, we saw that most often, vendor documentation included language that promotes their products, focusing primarily on positive characteristics where the artifact primarily serves as a way for vendors to communicate organizational benefits to governments. Here, transparency is framed less as accountability or disclosure and more as a way to emphasize efficiency, innovation, alignment with values, and broad applicability. These factsheets highlight value propositions, organizational commitments, and positive social impacts. 

Vendors that exhibit factsheet language reflecting showcasing tendencies share a few common features. First, they tend to emphasize benefits and value, often using quantitative claims to strengthen their claims. Often, vendors will highlight the substantial gains that are possible as immediate benefits. For example, when asked about performance metrics, one vendor offers a “70 to 90 percent reduction in report-writing time” or the ability to “reduce [tasks] to around 2-7 minutes.” These claims generally emphasize the potential value that agencies can tap to improve business process efficiencies and workflows. 

Second, these factsheets communicate their systems in a way that emphasizes the breadth of domains they address. In this way, vendors often describe their tools as “built for use across all levels of the public sector” or having “troves of rich performance data organized by every departmental domain for every state and local government,” where they position their systems as universally adaptable and applicable rather than specialized or constrained. This idea of uncapped robustness and expansive coverage is further illustrated by infrastructure descriptions such as deployment on “a scalable and elastic cloud-based platform to ensure optimal performance and unlimited quantity of records.” Claims like these may aim to help vendors establish credibility and promote alignment in competitive markets. 

Finally, these factsheets frequently provide reassurances that values alignment and regulation compliance can be accommodated by vendors without further agency management. This documentation implies responsible AI commitments in broad terms, for example stating that “all training is done on publicly available data” or that updates are conducted “frequently,” signalling that these concerns may be addressed by the vendor. When foundation models are involved, this documentation sometimes cites upstream assurances (e.g., “OpenAI continually refines and updates their models with legally obtained and fully licensed data”) as indirect evidence of their own system’s trustworthiness. These value-oriented claims aim to reinforce legitimacy and reassure agencies that additional oversight or governance measures are unnecessary. 

\xhdr{Factsheets as quality assessment}
Another major (and competing) goal focuses on using the factsheet as a mechanism for quality assessment. Given a set of needs, requirements, or responsible AI standards, some readers must begin to assess whether a particular system meets their agency’s needs. When agencies ask appropriate questions and vendors provide useful data and information, all stakeholders can work toward better understanding and evaluation, leading to better decision making. 
\textit{Interviews} This sentiment was present in both vendor and agency conversations in many different contexts. In many cases, agencies argued that technical understanding was important to decision makers throughout the procurement process. For example, one agency employee mentioned the importance of “Data, data, data, data, and where it's stored is first and foremost.” and another that “Data protection is huge for us because we're local government, and so we like to see certifications like SOC II”. While another focused on the importance of good model information, saying “I asked which model they are using and there's a section about the training data, and I am asking whether or not this model or product is going to continue to train on the data [from the city] that was ingested.”

This goal was emphasized by vendors as well. They believe that better evaluations lead to better solution alignment. For example, when talking about agency decision making, Vendor Participant 3 said: 
\begin{quote}
    “I know they're not asking the right questions, … so I think from the procurement lens, I would love to just be able to help them properly evaluate a tool … [We would] encourage people to test things that are out in the wild. I would encourage them to test a certain way. We've noticed a lot of our competitors don't have the same ability to contextualize information as we do… I think that it's those types of detailed things that I think if someone doesn't know how to evaluate, they're not going to ask that question.”
\end{quote}

It is important to note that these sentiments aren't exclusively aligned with specific stakeholder groups. Some vendors expressed genuine interest in providing meaningful quality assessments and clearer technical information, while a few agencies admitted they were not yet equipped to perform in-depth evaluations. This suggests that the challenge is not just differing incentives, but also highlights differing capacities and literacies across organizations.

\textit{Documentation}
A small set of factsheets emphasized this more technical approach where they focused on providing quantifiable information that highlighted the technical aspects of the system. These evaluation-centric factsheets describe internal testing regimes, data practices, system boundaries, and performance metrics. An evaluation-focused approach lends itself to expectations for thorough reviews and useful information for decision making. These factsheets can be used for better accountability, demonstrate adherence to standards, readiness for deployment, or compliance with responsible AI principles. But in practice, we found that the wide range of responses may highlight the need for further prompt refinement to better accommodate quality assessment. 

Factsheets that adopt an evaluation-oriented approach distinguish themselves through a more technical, evidence-forward framing. These documents provide quantifiable indicators of system performance, often referencing accuracy scores, precision/recall, or false-positive rates. Claims such as “demonstrates high accuracy based on internal validation tests,” “85\%+ F1 score is our general target,” or commitments to “continuous evaluation and refinement” express technical maturity and efficiency, while others provided qualitative statements about internal validation processes. We saw wide variation in disclosures. On one end of the range, we saw concrete, reproducible indicators that include explanations of the metrics, current performance, and target performance: 

\begin{quote}
    “Faithfulness: This checks how reliable the solution is in avoiding false or made-up information. In other words, it ensures the answers are based on real facts and knowledge. Current: 83\% Target: 96\%; Precision: This assesses whether the solution provides answers that are not only correct and accurate but also aligned with what the question specifically asks for. Current: 79.5\% Target: 90\%; Recall: This measures how much relevant information from all the available facts is successfully included in the answers, ensuring important details aren’t left out. Current: 89.4\% Target: 90\%.”
\end{quote} While on the other end of the spectrum, we found generalized claims about “high accuracy” or “ongoing refinement” with no current scores and no way to assess performance. This variability highlights that while a few vendors offered disclosures that could ground a more structured evaluation, most vendors provided information that was insufficient for comparative or context-appropriate assessment.

Relatedly, many evaluation-oriented factsheets frequently describe internal testing regimes, such as bias testing workflows, quality assurance processes, or audit checkpoints. These descriptions can provide meaningful insight into the maturity of internal governance practices. Here again we find wide variation in specificity where for example some vendors outline concrete procedures, while others mention their internal reviews without elaboration. For example one factsheet highlights their internal processes by mentioning “[good process]”, while another provides a much shorter explanation, with a complete entry only saying “We manage bias by a mandatory human review process.”. 

There were also many factsheets that chose to report metrics associated with business use cases as opposed to AI or ML technical performance metrics as mentioned in the previous section. These evaluative approaches emphasize the interpretability of the factsheet and goals that support evaluation of the use case rather than the model, often framed as evidence of system value rather than technical capability. Some factsheets instead signal evaluation and value by referencing external standards or frameworks (e.g., NIST AI RMF, SOC II, or ISO standards) as indicators of alignment with best practices. For example, nearly \% of the factsheets cite compliance with SOC II requirements, a security framework that specifies how organizations should protect customer data from unauthorized access, security incidents, and other vulnerabilities established by the American Institute of Certified Public Accountants (AICPA). 

Overall, evaluation-oriented factsheets demonstrate a meaningful shift toward documentation as evidence, with clear potential for supporting quality assessment, procurement due diligence, and responsible AI oversight. These documents could provide a clear path toward verifiable transparency, but these artifacts need a standardized prompt structure and additional support for informed decision-making or comparative assessment. 

\xhdr{Factsheets as building productive long term relationships}
Both vendors and agencies also recognized the potential of factsheets as a way to start building productive long term relationships. In this way, we found that documentation plays a role much earlier in the procurement process to facilitate strengthening the relationship between the vendor and agency as early as possible. Even when participants doubted that a static document could capture everything necessary for evaluation, they valued it as a shared reference point to build shared understanding and trust. 
\textit{Interviews}One agency participant’s perspective best demonstrated this idea through their intentional use of the Factsheet as a tool for building trust and investing in better partnerships. In describing a conversation one agency had with a vendor, they said “Because [the AI vendor] felt safe in the relationship with us, they knew it wasn't a "gotcha". It was "do the best you can". So they did, and their answer wasn't perfect,” and they went on to talk about how the agency and vendor built a better system through continued collaboration and communication. This sentiment was also echoed by vendors. For instance, one vendor really reflected on the value of sharing good information with agencies, saying “Overall, I think [the factsheet is] beneficial. Again, the more you share, it's been my experience in state and local government, the better opportunity you'll have.”

This view reframes transparency documentation not as an endpoint, but as an interactional resource. In this way, it becomes a way of establishing mutual understanding and literacy across organizational and disciplinary divides. This perspective sees the factsheet as just one document that establishes common ground and common language within the context of an ongoing relationship. Here there are continued opportunities to discuss and build upon what is written to provide a final solution that is more perfectly aligned with the needs of the government and the capabilities of the vendor. 

We found that factsheets sometimes serve as both symbolic and practical tools for building trust. They are symbolic in that they signal a commitment to responsible practice, and practical in that they provide a common vocabulary for discussing risks, tradeoffs, and governance expectations.

\textit{Documentation}
We also saw that many of the factsheets served well as tools to facilitate early communication rather than providing definitive or comprehensive information. In our interviews, vendors and agencies alike framed these documents as living artifacts, meant to evolve alongside procurement conversations or pilot deployments. This approach frames factsheets as a way to surface expectations, clarify misunderstandings, and build shared vocabulary and trust between vendors and government buyers. In our analysis, initial relationship building was the default approach assigned to factsheets if showcasing or evaluation language were not present. 

Factsheets that are used to start a conversation have a few shared characteristics. These factsheets typically provide broad summaries of system purpose, functionality, and intended use, without too much technical depth. Instead of providing detailed responses, vendors will include statements that indicate the need and ability for further information and refinement. This can prompt agencies to articulate their priorities and constraints earlier in the process. For example, one complete response to a prompt on poor conditions stated, “It totally depends on the use case,” which may signal that the vendor is awaiting further inputs before describing model behavior or setting expectations. 

This approach supports some procurement related goals such as early scoping, expectation-setting, and identifying potential points of concern. It allows agencies to test alignment at a conceptual level and reduces the risk of prematurely committing to or locking in technical specifications. But it also means that early factsheet versions may need further refinement before they can meaningfully support formal governance processes like risk assessments, comparative evaluations, or rule-based compliance checks alone.

\bkedit{
\xhdr{Applying the CDT Rubric (Should have a better name)}
To complement our qualitative analysis of how factsheets are completed and used in practice, we conducted an exploratory quantitative assessment of the full set of completed GovAI factsheets. 
For this, we used a new CDT rubric designed for evaluating transparency in public-sector AI systems called. 
The \textit{Framework for Assessing AI Transparency in the Public Sector}[ref] operationalizes governance-oriented transparency expectations across several dimensions, including governance structures, evaluation and testing, training data and methodologies, and use and context limitations. 
Applying this rubric allowed us to examine how the observed documentation practices align with emerging policy-facing standards for AI transparency, without assuming vendor intent or compliance motivations.

\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{source//figs/CDT_scores.pdf}
    \caption{While vendors frequently provide meaningful information about intended use and contextual limitations, disclosures relevant to evaluation, governance, and training data remain sparse. This asymmetry underscores the mismatch between expectations that factsheets function as evaluation tools and the realities of voluntary, public-facing documentation, reinforcing their practical role as relational, early-stage governance artifacts.}
    \label{fig:rubric_scores}
\end{figure}

Figure\ref{fig:rubric_scores} summarizes the aggregate distribution of scores across four rubric dimensions. The results reveal a consistent pattern. 
Here we see that factsheets scored relatively high on Use and Context Limitations, with a majority of submissions receiving medium or high scores, indicating that vendors frequently describe intended use cases, deployment contexts, and high-level constraints. 
In contrast, the remaining dimensions received predominantly low scores. In particular, no factsheets achieved a top score in Evaluation and Testing, and only a small number received high scores in Governance Structures or Training Data. 
These results suggest that while factsheets often provide contextual and descriptive information, they much less frequently include the detailed, verifiable technical or governance information needed to support systematic quality assessment or assurance.
}

\subsection{Challenges and Structural Obstacles to Factsheet Efficacy (Use?)}
Although factsheets are often seen as flexible tools that can simultaneously support procurement through a wide range of functions such as showcasing and quality assessment, our findings suggest that these multiple goals frequently work at cross purposes. Since different stakeholders approach the factsheet with different goals, it may result in interactions where no one fully gets what they need from these partnerships. Often, vendors attempt to present their systems in ways that highlight value and minimize legal exposure while agencies hope to obtain actionable technical insight to evaluate risk, while the template attempts to support these differing functions in one combined document. This multiplicity of purposes can create tensions before any question is even answered. 

These tensions are compounded by misaligned incentives. Right now, there are few meaningful incentives that would encourage vendors to overcome their concerns and provide more detailed or candid disclosures. At the same time, the disincentives to disclosure are significant. Legal exposure under FOIA/PRA, loss of competitive advantage, uncertain intellectual-property boundaries, and organizational limits on what information is even known or knowable within complex supply chains all disincentivize vendors from fully sharing information about their systems. So even when vendors and agencies explicitly agree on a shared purpose, such as supporting quality assessment or enabling more responsible procurement, these structural disincentives make full disclosure difficult, and in some cases impossible.

It is important to understand these challenges to characterize what factsheets currently do, and for clarifying what they can realistically achieve. Many of the issues raised below reflect broader characteristics of the public-sector AI ecosystem and its relationship to the private sector rather than shortcomings of any particular vendor or agency. This also means they are unlikely to be resolved solely through template revisions or better guidance. Instead, these obstacles reveal deeper structural dynamics that shape how transparency can be negotiated in practice. We can examine these challenges from the perspective of both vendors and agencies to better understand why written documentation struggles to achieve specific goals of the entities involved, and to explore how future governance mechanisms might better address or circumvent these constraints.

\xhdr{Competing Purposes and Communication Breakdowns}
One recurring source of friction exists where vendors and agencies enter the procurement process with fundamentally different expectations about what the factsheet is meant to accomplish. Even when both parties participate in good faith, misalignment between showcasing and evaluation goals can lead to misunderstandings. Agencies often approach the factsheet hoping to assess real-world limitations, failure modes, or compliance with technical and contextual requirements (quality assessment). Vendors, meanwhile, frequently view the same document as an opportunity to highlight value propositions, signal usability, or demonstrate potential efficiency gains (showcasing).

These competing purposes make it easy for communication to break down. For example, one agency participant expressed frustration when a vendor provided high-level narratives rather than the quantitative metrics the agency considered foundational for determining technical suitability. From the agency perspective, the omission of specifics felt evasive, like being pitched by a “snake oil salesman.” But from the vendor’s perspective, leading with impact-oriented examples or time-savings estimates is often a reasonable way to position their system. Both were answering the question of “What does your system do?”, but with different goals in mind. These tensions illustrate how the factsheet’s multi-purpose form can unintentionally muddy expectations instead of clarifying them.

\xhdr{Information Sensitivity, Public Disclosure, and Competitive Risk}
Vendors described substantive structural and legal constraints that shaped what they felt comfortable sharing. Many expressed strong concerns about intellectual property protection, competitive disadvantage, and the implications of the Freedom of Information Act (FOIA). For vendors without large legal teams or mature compliance infrastructure, the idea that there is no such thing as private written information shared with the government was a common source of anxiety. As one vendor mentioned “everything's FOIAed, so, that's always in the back of your mind that what you're putting in, could get right into your competitor's hands… that's certainly a factor that's in your mind as you're completing things.” Participants worried that providing too much technical detail could expose proprietary approaches and that they viewed prompt engineering strategies, internal heuristics, or fine-tuning methods as core to their competitive edge. As one vendor put it, “The things I wouldn't want to put [on the Factsheet] would be our methods into prompting, our methods … that's our edge … we've had people ask about that stuff, and we just tell them, hey, this is proprietary.”

Vendors described specific scenarios in which they imagined competitors using publicly available documentation to reverse-engineer system logic or extract architectural insights. For some companies, the risk of involuntary public disclosure was perceived as existential. From this perspective, the public and voluntary nature of the factsheets interacts directly with incentives. In a context where transparency may weaken competitive positioning, vendors often feel that they lack compelling reasons to disclose details that could be used against them. These concerns may help explain why many responses gravitate toward general descriptions, high-level claims, or business-oriented descriptions rather than technical specificity, even when vendors are supportive of transparency

\xhdr{Opacity and Responsibility Gaps Within AI Supply Chains}
A third set of obstacles stems from the growing complexity of AI supply chains. Many vendors do not build models end-to-end, instead, they integrate or fine-tune foundation models developed by large upstream providers. As a result, they often lack visibility into pretraining datasets, licensing arrangements, or model development practices, even if they wanted to disclose them. In these cases, the issue is not necessarily a reluctance to share but a perceived inability to access the requested information. For systems built on top of APIs such as GPT-4 or other foundation models, vendors frequently explained that they could not provide details about training data provenance or model internals because that information does not exist in a form they can access.

Vendors responded to this gap in several ways. Some used the factsheet to clarify the limits of their responsibility, emphasizing that performance depends heavily on downstream factors such as data quality, prompt formulation, or customer deployment context. Others described themselves as integrators rather than creators, highlighting the mismatch between what the template implicitly assumes (full system visibility) and what their actual role permits. In multiple cases, vendors mentioned that there should be default “drop down style menus” to answer many factsheet questions because “everyone is using ChatGPT.” One vendor specified this further saying “it's almost like you'd want to be able to check ‘OpenAI GPT-4o’ or ‘Google Gemini 3.5’ so that there's a boilerplate [answer] that exists, rather than reinventing the wheel. For those of us that are leveraging commercial LLMs that makes more sense.” This dynamic reflects broader shifts in the AI market. As more vendors build products atop foundation models, they believe that the onus for meaningful transparency moves upstream, often out of reach of those asked to complete the documentation.

From a governance perspective, this raises important questions about what transparency can realistically look like when no single party has full system-level knowledge. The factsheet’s design assumes a level of centralized control that is increasingly rare. Vendors may be willing to be transparent, but the structure of the market and the incentives of upstream providers constrains what can (or will) be disclosed.

% \xhdr{Factsheets as showcasing value added} Across interviews with both vendors and public-sector practitioners, a dominant way of understanding the factsheet was as an opportunity to showcase the value a system provides for a particular problem. Rather than framing the document primarily as a vehicle for technical disclosure or risk assessment, many participants described it as a space to communicate benefits, differentiation, and practical relevance. This orientation toward showcasing value was visible not only in how stakeholders talked about the factsheet, but also in how vendors completed it in practice.

% Vendors frequently described the factsheet as a chance to highlight what makes their system attractive in a competitive market. One participant emphasized wanting “more opportunity to showcase what differentiates [our] product from the competition,” while another framed the factsheet as a way to gain “any exposure, especially for small companies,” explaining their desire to “maximize the eyeballs” that ultimately see it. Notably, this orientation was not limited to vendors. Agency interviewees often echoed similar priorities, emphasizing outcomes and problem-solving over technical detail. As one public-sector participant put it: “We don't want to get technical about how [the AI] works. I don't care about the programming, or what program you use, but how does it solve the problem” (AP).

% This shared focus on value and fit was reflected clearly in the content of completed factsheets. Across the corpus, vendor responses frequently emphasized positive characteristics and anticipated benefits, positioning the artifact less as a mechanism for accountability or scrutiny and more as a promotional document oriented toward efficiency, innovation, and alignment with public-sector values. In this framing, transparency is operationalized through accessible narratives about what a system enables an agency to do, rather than through detailed disclosures about how the system is built or governed.

% One recurring pattern involved the use of quantitative claims to underscore value propositions. When responding to prompts about system performance, vendors often highlighted efficiency gains, such as a “70 to 90 percent reduction in report-writing time” or the ability to “reduce [tasks] to around 2–7 minutes.” These claims foreground immediate, tangible improvements to workflows and business processes, reinforcing the idea that the system’s primary relevance lies in its practical impact rather than its technical design.

% A second pattern was the emphasis on breadth and generalizability. Many factsheets described systems as broadly applicable across agencies, jurisdictions, or use cases, using language such as “built for use across all levels of the public sector” or offering “troves of rich performance data organized by every departmental domain for every state and local government.” Infrastructure descriptions similarly highlighted scalability and expansiveness, for example noting deployment on “a scalable and elastic cloud-based platform to ensure optimal performance and unlimited quantity of records.” These claims position systems as robust and universally adaptable, reinforcing credibility while minimizing the appearance of contextual constraints.

% Finally, value-oriented disclosures frequently included reassurances about values alignment and regulatory compliance, often framed as vendor-managed concerns. Factsheets commonly asserted that “all training is done on publicly available data” or that system updates occur “frequently,” signaling that governance and oversight issues are already being addressed. In cases involving foundation models, vendors sometimes cited upstream assurances—such as statements that “OpenAI continually refines and updates their models with legally obtained and fully licensed data”—as indirect evidence of their own system’s trustworthiness. Together, these claims work to reassure agencies that additional scrutiny or governance intervention may be unnecessary.

% \xhdr{Factsheets as quality assessment} A second major—and often competing—goal articulated by participants was the use of factsheets as mechanisms for quality assessment. In this framing, the factsheet is expected to support judgments about whether a system meets an agency’s technical, operational, or responsible AI requirements. When agencies can ask appropriate questions and vendors can provide meaningful technical information, the factsheet is imagined as a tool that enables better evaluation, comparison, and ultimately, better procurement decisions.

% This expectation was voiced repeatedly in interviews with both agency staff and vendors. Agency participants emphasized the importance of access to concrete technical and governance information throughout the procurement process. Several pointed to data practices and security as foundational concerns, with one participant stressing the primacy of “data, data, data, data, and where it's stored is first and foremost,” and another highlighting the importance of recognized certifications, noting that “data protection is huge for us because we're local government, and so we like to see certifications like SOC II.” Others focused more narrowly on model behavior and lifecycle risks, describing the need to understand training data and downstream use, such as whether a system “is going to continue to train on the data [from the city] that was ingested.”

% Vendors also articulated strong support for more rigorous evaluation, often framing it as a way to improve alignment and avoid poor-fit deployments. One vendor expressed frustration that agencies often “aren’t asking the right questions,” arguing that procurement processes would benefit from better guidance on how to evaluate tools in practice. As they explained, encouraging agencies to test systems “a certain way” could surface meaningful differences between products—differences that might otherwise be missed when evaluative capacity is uneven or underdeveloped. Notably, these perspectives cut across stakeholder groups: while some vendors expressed genuine interest in providing deeper technical detail, several agency participants acknowledged that they lacked the expertise or institutional capacity to conduct in-depth assessments. This suggests that challenges around quality assessment stem not only from misaligned incentives, but also from uneven literacies and evaluative resources across organizations.

% These aspirations toward evaluative use were reflected, unevenly, in the completed factsheets. A small subset adopted a distinctly evaluation-oriented approach, providing technical, evidence-forward disclosures about system performance, testing regimes, data practices, and governance processes. These factsheets included quantifiable metrics, references to internal validation procedures, and explicit descriptions of system boundaries, positioning the document as a source of evidence rather than promotion. In principle, such disclosures could support accountability, demonstrate readiness for deployment, and inform responsible AI oversight.

% In practice, however, we observed substantial variation in the depth, clarity, and reproducibility of evaluative information. Some vendors provided detailed performance metrics accompanied by explanations, current scores, and target benchmarks. For example, one factsheet reported multiple evaluation dimensions—such as faithfulness, precision, and recall—each with defined meanings, current performance levels, and explicit targets. These disclosures offer a rare glimpse into how a factsheet might function as a foundation for structured assessment.

% At the other end of the spectrum, many factsheets relied on generalized claims of “high accuracy,” “robust performance,” or “ongoing refinement,” without providing metrics, context, or baselines. Even when evaluation was mentioned, it was often difficult to assess what had been tested, under what conditions, or with what implications for deployment. This variability mirrors the tensions expressed in interviews: while stakeholders widely endorse the idea of evaluation, the information provided is often insufficient to support comparative or context-sensitive judgments.

% A similar pattern emerged in disclosures about internal testing and governance practices. Some factsheets described bias testing workflows, quality assurance checkpoints, or audit processes in concrete terms, offering insight into organizational maturity and oversight. Others referenced internal reviews only briefly or abstractly, such as stating that “bias is managed through a mandatory human review process,” without further elaboration. These abbreviated disclosures gesture toward evaluative intent but provide little basis for meaningful scrutiny.

% Finally, many factsheets framed evaluation through business-oriented metrics or external certifications rather than AI- or model-specific performance indicators. In these cases, evaluation was oriented toward use-case success, operational efficiency, or organizational compliance, rather than technical behavior. References to frameworks such as SOC II, ISO standards, or the NIST AI Risk Management Framework were frequently used as signals of trustworthiness and alignment with best practices. While such references may be useful heuristics for risk screening, they often substitute for, rather than complement, detailed system-level evaluation.

% \xhdr{Factsheets as building productive long-term relationships} Beyond showcasing value or supporting quality assessment, both vendors and agencies described factsheets as tools for initiating and sustaining productive long-term relationships. In this framing, documentation operates earlier in the procurement lifecycle, helping to establish trust, shared understanding, and communicative footing before formal evaluation or contractual commitment takes place. Even participants who were skeptical that a static document could support rigorous assessment emphasized its value as a shared reference point—something that makes subsequent dialogue easier, safer, and more productive.

% This perspective was articulated most clearly in interviews where participants reflected on trust-building dynamics between vendors and agencies. One agency participant described how a sense of relational safety fundamentally shaped disclosure practices: “Because [the AI vendor] felt safe in the relationship with us, they knew it wasn't a ‘gotcha.’ It was ‘do the best you can.’ So they did, and their answer wasn't perfect.” In this account, the factsheet did not function as a compliance artifact or evaluative gatekeeper, but as an entry point into collaborative problem-solving. The agency and vendor were able to iteratively improve the system through continued communication, using the factsheet as a starting scaffold rather than a final judgment.

% Vendors echoed this relational framing, often linking openness to long-term opportunity rather than immediate transactional gain. One vendor reflected that “the more you share, it’s been my experience in state and local government, the better opportunity you’ll have,” emphasizing that early transparency can signal good faith and lay the groundwork for durable partnerships. These interview accounts collectively position transparency documentation not as an endpoint, but as an interactional resource—one that helps bridge organizational, disciplinary, and expertise divides by establishing shared language and expectations.

% This relational role was also visible in the completed factsheets themselves. Many documents appeared designed less to provide definitive or exhaustive information and more to facilitate early-stage communication. Vendors and agencies alike described factsheets as living artifacts, intended to evolve alongside procurement conversations, pilot deployments, or scoping exercises. In our analysis, when factsheets did not strongly exhibit showcasing or evaluation-oriented language, they most often defaulted to this relationship-building function.

% Factsheets oriented toward relationship-building share several common characteristics. They typically provide high-level descriptions of system purpose, functionality, and intended use, while deliberately avoiding deep technical specificity. Rather than offering definitive answers, vendors often include language that signals openness to further discussion or refinement. For example, one response to a prompt about poor operating conditions simply stated, “It totally depends on the use case,” effectively inviting agencies to articulate their priorities and constraints before committing to particular claims about system behavior. While such responses may appear vague when viewed through an evaluative lens, they can serve an important relational purpose by keeping the conversation open.

% This approach supports several procurement-relevant goals, including early scoping, expectation-setting, and the identification of potential areas of concern. By enabling agencies to assess conceptual fit without prematurely locking in technical specifications, relationship-oriented factsheets can reduce early-stage risk and misalignment. At the same time, this use highlights an important limitation: factsheets that function well as conversation starters often lack the detail needed to support downstream governance activities such as formal risk assessment, comparative evaluation, or rule-based compliance checks.

% \subsection{Challenges and Structural Obstacles to Factsheet Efficacy}
% Although factsheets are often seen as flexible tools that can simultaneously support procurement through a wide range of functions such as showcasing and quality assessment, our findings suggest that these multiple goals frequently work at cross purposes. Since different stakeholders approach the factsheet with different goals, it may result in interactions where no one fully gets what they need from these partnerships. Often, vendors attempt to present their systems in ways that highlight value and minimize legal exposure while agencies hope to obtain actionable technical insight to evaluate risk, while the template attempts to support these differing functions in one combined document. This multiplicity of purposes can create tensions before any question is even answered. 

% These tensions are compounded by misaligned incentives. Right now, there are few meaningful incentives that would encourage vendors to overcome their concerns and provide more detailed or candid disclosures. At the same time, the disincentives to disclosure are significant. Legal exposure under FOIA/PRA, loss of competitive advantage, uncertain intellectual-property boundaries, and organizational limits on what information is even known or knowable within complex supply chains all disincentivize vendors from fully sharing information about their systems. So even when vendors and agencies explicitly agree on a shared purpose, such as supporting quality assessment or enabling more responsible procurement, these structural disincentives make full disclosure difficult, and in some cases impossible.

% It is important to understand these challenges to characterize what factsheets currently do, and for clarifying what they can realistically achieve. Many of the issues raised below reflect broader characteristics of the public-sector AI ecosystem and its relationship to the private sector rather than shortcomings of any particular vendor or agency. This also means they are unlikely to be resolved solely through template revisions or better guidance. Instead, these obstacles reveal deeper structural dynamics that shape how transparency can be negotiated in practice. We can examine these challenges from the perspective of both vendors and agencies to better understand why written documentation struggles to achieve specific goals of the entities involved, and to explore how future governance mechanisms might better address or circumvent these constraints.

% \xhdr{Information Sensitivity, Public Disclosure, and Competitive Risk}
% Vendors described substantive structural and legal constraints that shaped what they felt comfortable sharing. Many expressed strong concerns about intellectual property protection, competitive disadvantage, and the implications of the Freedom of Information Act (FOIA). For vendors without large legal teams or mature compliance infrastructure, the idea that there is no such thing as private written information shared with the government was a common source of anxiety. As one vendor mentioned “everything's FOIAed, so, that's always in the back of your mind that what you're putting in, could get right into your competitor's hands… that's certainly a factor that's in your mind as you're completing things.” Participants worried that providing too much technical detail could expose proprietary approaches and that they viewed prompt engineering strategies, internal heuristics, or fine-tuning methods as core to their competitive edge. As one vendor put it, “The things I wouldn't want to put [on the Factsheet] would be our methods into prompting, our methods … that's our edge … we've had people ask about that stuff, and we just tell them, hey, this is proprietary.”

% Vendors described specific scenarios in which they imagined competitors using publicly available documentation to reverse-engineer system logic or extract architectural insights. For some companies, the risk of involuntary public disclosure was perceived as existential. From this perspective, the public and voluntary nature of the factsheets interacts directly with incentives. In a context where transparency may weaken competitive positioning, vendors often feel that they lack compelling reasons to disclose details that could be used against them. These concerns may help explain why many responses gravitate toward general descriptions, high-level claims, or business-oriented descriptions rather than technical specificity, even when vendors are supportive of transparency

% \xhdr{Opacity and Responsibility Gaps Within AI Supply Chains}
% A third set of obstacles stems from the growing complexity of AI supply chains. Many vendors do not build models end-to-end, instead, they integrate or fine-tune foundation models developed by large upstream providers. As a result, they often lack visibility into pretraining datasets, licensing arrangements, or model development practices, even if they wanted to disclose them. In these cases, the issue is not necessarily a reluctance to share but a perceived inability to access the requested information. For systems built on top of APIs such as GPT-4 or other foundation models, vendors frequently explained that they could not provide details about training data provenance or model internals because that information does not exist in a form they can access.

% Vendors responded to this gap in several ways. Some used the factsheet to clarify the limits of their responsibility, emphasizing that performance depends heavily on downstream factors such as data quality, prompt formulation, or customer deployment context. Others described themselves as integrators rather than creators, highlighting the mismatch between what the template implicitly assumes (full system visibility) and what their actual role permits. In multiple cases, vendors mentioned that there should be default “drop down style menus” to answer many factsheet questions because “everyone is using ChatGPT.” One vendor specified this further saying “it's almost like you'd want to be able to check ‘OpenAI GPT-4o’ or ‘Google Gemini 3.5’ so that there's a boilerplate [answer] that exists, rather than reinventing the wheel. For those of us that are leveraging commercial LLMs that makes more sense.” This dynamic reflects broader shifts in the AI market. As more vendors build products atop foundation models, they believe that the onus for meaningful transparency moves upstream, often out of reach of those asked to complete the documentation.

% From a governance perspective, this raises important questions about what transparency can realistically look like when no single party has full system-level knowledge. The factsheet’s design assumes a level of centralized control that is increasingly rare. Vendors may be willing to be transparent, but the structure of the market and the incentives of upstream providers constrains what can (or will) be disclosed.

% \xhdr{FactSheets as quality assessment}

% \color{brown}\njcomment{TODO}
% A second major goal articulated by participants was the use of FactSheets as mechanisms for quality assessment. In this framing, the FactSheet is expected to support judgments about whether a system meets an agency’s technical, operational, or responsible AI requirements. When agencies can ask appropriate questions and vendors can provide meaningful technical information, the FactSheet is imagined as a tool that enables evaluation, comparison, and more informed procurement decisions.

% This expectation was voiced repeatedly in interviews with both agency staff and vendors. Agency participants emphasized the importance of access to concrete technical and governance information, particularly around data practices and security. Several described data storage and protection as foundational concerns, with one participant stressing the primacy of “data, data, data, data, and where it's stored is first and foremost,” and another highlighting the importance of recognized certifications, noting that “data protection is huge for us because we're local government, and so we like to see certifications like SOC II.” Others focused on model behavior and lifecycle risks, such as whether a system “is going to continue to train on the data [from the city] that was ingested.”

% Vendors likewise expressed support for more rigorous evaluation, often framing it as a way to improve alignment and avoid poor-fit deployments. One vendor argued that agencies often “aren’t asking the right questions,” suggesting that clearer evaluative guidance and more structured testing could surface meaningful differences between systems. At the same time, several agency participants acknowledged limited institutional capacity or technical expertise to conduct in-depth assessments. Together, these perspectives suggest that challenges around quality assessment stem not only from misaligned incentives, but also from uneven evaluative literacies and resources across organizations.

% These aspirations toward evaluative use were reflected unevenly in the completed FactSheets. A small subset adopted a distinctly evaluation-oriented approach, providing technical, evidence-forward disclosures about system performance, testing regimes, data practices, and governance processes. These FactSheets included quantifiable metrics, references to internal validation procedures, and explicit descriptions of system boundaries, positioning the document as a source of evidence rather than promotion. For example, one FactSheet reported multiple evaluation dimensions such as faithfulness, precision, and recall, each with defined meanings, current performance levels, and target benchmarks, illustrating how FactSheets might support structured assessment.

% More commonly, however, FactSheets relied on generalized claims such as “high accuracy,” “robust performance,” or “ongoing refinement,” without providing metrics, baselines, or testing context. Even when evaluation was mentioned, it was often unclear what had been assessed or how results should be interpreted. Similar patterns appeared in disclosures about governance and testing practices: some FactSheets described bias testing or quality assurance workflows in concrete terms, while others gestured vaguely toward internal review processes without sufficient detail to enable scrutiny.

% Finally, many FactSheets framed evaluation through business-oriented metrics or external certifications rather than AI- or model-specific performance indicators. References to frameworks such as SOC II, ISO standards, or the NIST AI Risk Management Framework were frequently used as signals of trustworthiness and compliance. 
% % While such references may function as useful heuristics for initial risk screening, they often substitute for, rather than complement, detailed system-level evaluation.

% \xhdr{FactSheets as quality assessment}
% A second major goal articulated by both governments and vendors was the use of FactSheets as tools for quality assessment. In this framing, documentation is expected to support judgments about whether a system is fit for a particular public-sector context: whether it meets an agency’s technical, operational, legal, or responsible AI requirements, and whether its risks are acceptable given the intended use.
% Importantly, participants described quality assessment not as a single metric or threshold, but as a process that allows agencies to decide for themselves what is “good enough,” rather than relying solely on vendor assurances that a system is safe, accurate, or effective. 
% Good quality assessment extends well beyond the “performance evaluation” portions of the FactSheet. It includes the ability to anticipate potential failure modes, understand how and where risks may appear across the system lifecycle, and identify what mitigations or governance measures may be required prior to or during deployment. To support these judgments, agencies need sufficient information about how a system was designed, trained, evaluated, and maintained, as well as clarity about its intended and unsuitable contexts of use. In principle, disclosures about data practices, evaluation methods, robustness, system boundaries, and governance processes could all contribute to this broader form of assessment.

% This was voiced repeatedly in interviews. Agency participants emphasized the need for concrete technical and governance information, particularly around data provenance and responsible AI governance. 
% For example, one agency participant mentioned their emphasis on the RAI aspects of representation in training data, saying: "I'm always thinking about training data... and I know that this technology ethically puts women and people of color more at risk."
% Others focused on model behavior and lifecycle risks, such as whether a system “is going to continue to train on the data [from the city] that was ingested.” or how the vendor plans for the AI solution to change and evolve over a long term "roadmap". 
% Vendors, in turn, often expressed support for more rigorous evaluation, framing it as a way to differentiate products and avoid poor-fit deployments.
% At the same time, both groups acknowledged that agencies may lack the technical expertise or institutional capacity to interpret highly detailed disclosures, complicating the use of open-ended technical information for quality assessment.

% In practice, however, our analysis suggests that completed FactSheets rarely provide the kind of information needed to support meaningful quality assessment. While a small subset of FactSheets adopted an evaluation-oriented approach, providing specific performance metrics, describing testing regimes, or outlining governance workflows, most relied on high-level claims such as “high accuracy,” “robust performance,” or “ongoing refinement,” without sufficient detail to interpret what had been tested, under what conditions, or with what limitations. Even when evaluation was mentioned, responses often lacked baselines, contextual explanations, or decision-relevant implications.

% For an agency using the FactSheet for quality assessment, this level of vagueness substantially limits the document’s usefulness. For example, an agency attempting to choose between two systems cannot meaningfully compare claims of “high accuracy” without knowing how accuracy was measured, on what data, or relative to what standard. Similarly, statements that a system performs poorly only in undefined “edge cases” provide little guidance for anticipating whether those conditions are likely to occur in a specific deployment context. As a result, agencies are left without the information needed to assess tradeoffs, identify risks, or determine whether additional safeguards are required.

% This pattern was not limited to performance-related disclosures. Similar gaps appeared in responses about robustness, optimal and poor operating conditions, data dependencies, and governance practices. While some vendors offered concrete descriptions, many provided generalized or conditional statements that gesture toward evaluation without enabling it. In these cases, FactSheets may signal that evaluation has occurred, but they do not provide the substance necessary for agencies to conduct their own assessments.

% Agencies also frequently cited certifications such as SOC II or ISO standards as examples of useful heuristics for assessing baseline organizational practices surrounding data security and compliance. However, in the absence of comparable certification regimes for other dimensions of AI quality such as model behavior, bias, or contextual suitability, FactSheets end up relying heavily on voluntary, open-ended technical disclosures. When those disclosures are sparse or difficult to interpret, the burden of quality assessment shifts back onto agencies that may lack the expertise or resources to fill in the gaps.

